High strehl and high contrast for the ELT instrument METIS -- Final design, implementation, and predicted performance of the single-conjugate adaptive optics system

The Mid-infrared ELT Imager and Spectrograph (METIS) is a first-generation instrument for the Extremely Large Telescope (ELT), Europe's next-generation 39 m ground-based telescope for optical and infrared wavelengths. METIS will offer diffraction-limited imaging, low- and medium-resolution slit spectroscopy, and coronagraphy for high-contrast imaging between 3 and 13 microns, as well as high-resolution integral field spectroscopy between 3 and 5 microns. The main METIS science goals are the detection and characterisation of exoplanets, the investigation of proto-planetary disks, and the formation of planets. The Single-Conjugate Adaptive Optics (SCAO) system corrects atmospheric distortions and is thus essential for diffraction-limited observations with METIS. Numerous challenging aspects of an ELT Adaptive Optics (AO) system are addressed in the mature designs for the SCAO control system and the SCAO hardware module: the complex interaction with the telescope entities that participate in the AO control, wavefront reconstruction with a fragmented and moving pupil, secondary control tasks to deal with differential image motion, non-common path aberrations and mis-registration. A K-band pyramid wavefront sensor and a GPU-based Real-Time Computer (RTC), tailored to the needs of METIS at the ELT, are core components. This current paper serves as a natural sequel to our previous work presented in Hippler et al. (2018). It includes updated performance estimations in terms of several key performance indicators, including achieved contrast curves. We outline all important design decisions that were taken, and present the major challenges we faced and the main analyses carried out to arrive at these decisions and eventually the final design. We also elaborate on our testing and verification strategy, and, last not least, comprehensively present the full design, hardware and software.

==> Common/metis_glossary.tex <==

%\setabbreviationstyle[acronym]{long-short}

% \newacronym[longplural={Frames per Second}]{fps}{FPS}{Frame per Second}
\newacronym[]{10ge} {10GE} {10 Gigabit per second Ethernet}
\newacronym[]{adc} {ADC}  {Atmospheric Dispersion Corrector}
\newacronym[]{adi}  {ADI}   {Angular Differential Imaging}
\newacronym[]{adr}  {ADR}   {Atmospheric Differential Refraction}
\newacronym[longplural={Active Galactic Nuclei}]{agn} {AGN}  {Active Galactic Nucleus}
\newacronym[]{ait}  {AIT}   {Assembly, Integration and Testing}
\newacronym[]{aiv}  {AIV}   {Assembly, Integration and Verification}
\newacronym[]{aka} {aka.}  {also known as}
\newacronym[]{alwfs}{ALWFS}{Asymmetric Lyot Wave Front Sensor}
\newacronym[]{ao}  {AO}   {Adaptive Optics}
\newacronym[]{aof}  {AOF}   {Adaptive Optics Facility}
\newacronym[]{aocs}  {AOCS}   {Adaptive Optics Control System}
\newacronym[]{aofcs}  {AO FCS}   {Adaptive Optics Function Control System}
\newacronym[]{aoocs}  {AO OCS}   {Adaptive Optics Observation Coordination System}
\newacronym[]{aop}  {AOP}   {AO pick-off mirror}
\newacronym[]{aosat}  {AOSAT}   {The adaptive optics simulation analysis tool(kit)}
\newacronym[]{ape} {APE}  {Active Phasing Experiment}
\newacronym[]{api} {API}  {Application Programming Interface}
\newacronym[]{app} {APP}  {Apodizing Phase Plate}
\newacronym[]{arr} {ARR}  {Acceptance Readiness Review}
\newacronym[]{avx2} {AVX2} {Advanced Vector Extensions 2}
\newacronym[]{cs} {CS}  {Control System}
\newacronym[]{cad} {CAD}  {computer-aided design}
\newacronym[]{ccs} {CCS}  {Central Control System}
\newacronym[]{cds} {CDS}  {Correlated Double Sampling}
\newacronym[]{cd} {CD}  {Control Deterministic}
\newacronym[]{cfo} {CFO}  {Common Fore-Optics Subsystem}
\newacronym[]{cfoccs} {CFO/CCS}  {Cold Central Structure}
\newacronym[]{cii} {CII}  {Core Integration Infrastructure}
\newacronym[]{ciao} {CIAO}  {Coudé Infrared Adaptive Optics}
\newacronym[]{cm}  {CM}   {Command Matrix}
\newacronym[]{cmcomp}  {CM Composer}   {Command Matrix Composer}
\newacronym[]{cog} {CoG}  {Center of Gravity}
\newacronym[]{compass} {COMPASS}  {COMputing Platform for Adaptive optics SystemS}
\newacronym[]{cots} {COTS}  {Commercial Off-The-Shelf}
\newacronym[]{cpu} {CPU}  {Central Processing Unit}
\newacronym[]{cry} {CRY}  {Cryostat Subsystem}
\newacronym[longplural={coefficients of thermal expansion}]{cte} {CTE}  {coefficient of thermal expansion}
\newacronym[]{cuda}{CUDA} {Nvidia Compute Unified Device Architecture}
\newacronym[]{cwfs} {CWFS}  {Curvature Wavefront Sensor}
\newacronym[]{cured} {CuReD}  {Cumulative Reconstructor with Domain Decomposition}
\newacronym[]{cvc} {CVC}  {Classical Vortex Coronagraph}

\newacronym[]{dac} {DAC}  {Digital to Analog Conversion}
\newacronym[]{dc} {DC}  {Detector Controller}
\newacronym[]{dcs} {DCS}  {Detector Control Software}
\newacronym[]{dds} {DDS}  {Data Distribution System}
\newacronym[]{ddt} {DTT}  {Data Display Tool}
\newacronym[]{det} {DET}  {(science) Detector Subsystem}
\newacronym[]{dfe} {DFE}  {Detector Front-End}
\newacronym[]{dho} {DHO}  {Differential High Order}
\newacronym[]{dhomon} {DHO Monitor} {Differential High Order Monitor}
\newacronym[]{dit} {DIT}  {Detector Integration Time (individual frame)}
\newacronym[]{dsm} {DSM}  {Deformable Secondary Mirror}

\newacronym[longplural={Deformable Mirrors}]{dm}  {DM}   {Deformable Mirror}
\newacronym[longplural={degrees of Freedom}, shortplural={DoF}]{dof} {DoF}  {Degree of Freedom}
\newacronym[]{dpm} {DPM}  {Data Product Manager}
\newacronym[]{dtt} {DTT}  {Differential tip-tilt}
\newacronym[]{dws} {DWS}  {Detector Workstation}

\newacronym[]{eapd}{eAPD}{electron avalanche photodiode array}
\newacronym[]{elt}{ELT}   {Extremely Large Telescope}
\newacronym[]{eelt}{E-ELT}{European Extremely Large Telescope}
\newacronym[]{es}{ES}{Edge Sensor}
\newacronym[]{eso} {ESO}  {European Southern Observatory}
\newacronym[]{ethercat}{EtherCAT}{Ethernet for Control Automation Technology}
\newacronym[]{e2e}{E2E}{end-to-end}

\newacronym[]{fcs} {FCS}  {Function Control System}
\newacronym[]{fdr} {FDR}  {Final Design Review}
\newacronym[]{fe} {FE}  {finite element}
\newacronym[]{fea} {FEA}  {Finite Element Analysis}
\newacronym[]{fir} {FIR}  {Finite Impulse Response Filter}
\newacronym[]{fits} {FITS}  {Flexible Image Transport System}
\newacronym[]{flao} {FLAO}  {First Light Adaptive Optics}
\newacronym[]{flop} {FLOP}  {Floating Point Operation}
\newacronym[]{flops} {FLOPS}  {Floating Point Operations per Second}
\newacronym[]{fov} {FoV}  {field of view}
\newacronym[]{fp} {FP}  {focal plane}
\newacronym[]{fpa} {FPA}  {focal plane array}
\newacronym[]{fprf} {FPRF}  {focal plane reference frame}
\newacronym[]{fpga} {FPGA}  {Field-Programmable Gate Array}
\newacronym[]{fps} {FPS}  {Focal Plane Sensor}
\newacronym[]{fpsgw} {FPS GW}  {Focal Plane Sensor Gateway}
\newacronym[]{freda} {FREDA}  {inFRaRED cAmera}
\newacronym[]{fsm} {FSM}  {\gls{field selector} Mirror}
\newacronym[]{fwhm} {FWHM}  {Full-Width-Half-Maximum}

\newacronym[]{gmt} {GMT}  {Giant Magellan Telescope}
\newacronym[]{gp} {GP}  {guide probe}
\newacronym[]{gpao} {GPAO}  {Guide Probe AO  (based on PFS Shack-Hartmann WFS)}
\newacronym[]{gpu} {GPU}  {Graphics Processing Unit}
\newacronym[]{gpgpu} {GPGPU}  {General-Purpose computing on Graphics Processing Units}
\newacronym[]{gravity} {GRAVITY}  {Second Generation VLTI instrument for precision narrow-angle astrometry and interferometric imaging}

\newacronym[]{gui} {GUI}  {Graphical User Interface}

\newacronym[]{h2rg}  {H2RG}   {HAWAII 2RG \gls{ir} \gls{fpa}}
\newacronym[]{harmoni}{HARMONI} {High Angular Resolution Monolithic Optical and Near-infrared Integral field spectrograph}
\newacronym[]{hbm}  {HBM}   {High Bandwidth Memory}
\newacronym[]{hbm2}  {HBM2}   {High Bandwidth Memory 2}
\newacronym[]{hci} {HCI}  {High-Contrast Imaging}
\newacronym[]{heeps} {HEEPS}  {High-contrast End-to-End Performance Simulator}
\newacronym[]{ho}  {HO}   {High Order}
\newacronym[]{howfs} {HO WFS}  {High Order Wavefront Sensor}
\newacronym[]{hrtc}  {HRTC}   {Hard Real-Time Core}
\newacronym[]{hw}  {HW}   {Hardware}

\newacronym[]{ice} {ICE}  {ZeroC Internet Communications Engine}
\newacronym[]{ics} {ICS}  {Instrument Control System}
\newacronym[]{icd} {ICD}  {Interface Control Document}
\newacronym[]{icar} {ICAR}  {Indexed Cryogenic Actuator for Rotation}
\newacronym[]{ide} {IDE}  {Integrated Development Environment}
\newacronym[]{if}  {I/F}  {interface}
\newacronym[]{iir} {IIR}  {Infinite Impulse Response Filter}
\newacronym[]{inf}  {IF}  {influence function}
\newacronym[]{ifu} {IFU}  {Integral Field Unit}
\newacronym[]{ip}  {IP}   {Internet Protocol}
\newacronym[]{ir}  {IR}   {Infrared}
\newacronym[]{im}  {IM}   {interaction matrix}
\newacronym[]{img}  {IMG} {Imager Subsystem}
\newacronym[]{ins} {INS}  {Instrument}
\newacronym[]{irq} {IRQ}  {Interrupt Request}
\newacronym[]{iwa} {IWA}  {inner working angle}

\newacronym[]{kpa} {KPA}  {Kernel Phase Analysis}
\newacronym[]{kpp} {KPI}  {Key Performance Indicator}
\newacronym[]{kl} {KL}  {Karhunen–Loève}

\newacronym[]{lbt} {LBT}  {Large Binocular Telescope}
\newacronym[]{lc}  {LC}   {Lucent Connector}
\newacronym[]{lci}  {LCI}   {Local Communication Infrastructure}
\newacronym[]{lcs} {LCS}  {Local Control System}
\newacronym[]{lesia} {LESIA}  {Laboratoire d'études spatiales et d'instrumentation en astrophysique, l'Observatoire de Paris}
\newacronym[]{lli} {LLI}  {long leadtime item}
\newacronym[]{lms} {LMS}  {L/M band Spectrograph Subsystem}
\newacronym[]{ln} {LINC-NIRVANA}  {Near infrared imaging instrument for the Large Binocular Telescope}
\newacronym[]{lo}  {LO}   {Low Order}
\newacronym[]{loo} {LOO}  {\gls{Low Order Optimisation}}
\newacronym[]{lwe} {LWE}  {low wind effect}
\newacronym[]{lowfs} {LO WFS}  {Low Order Wavefront Sensor}
\newacronym[]{ls} {LS}  {least-squares reconstructor}
\newacronym[]{lti} {LTI}  {Linear time-invariant system}
\newacronym[]{lu} {LU}    {Lens Unit}
\newacronym[]{lgs} {LGS}  {Laser Guide Star}
\newacronym[]{lqg} {LQG}  {Linear-quadratic-Gaussian}
\newacronym[]{lqi} {LQI}  {Linear-quadratic-Integral}
\newacronym[]{lt}  {LT}   {Launch Telescope}
\newacronym[]{ltao}{LTAO} {Laser Tomography Adaptive Optics}
\newacronym[]{m2c}  {M2C}   {modes-to-commands matrix}
\newacronym[]{mait}  {MAIT}   {Manufacturing, Assembly, Integration and Testing}
\newacronym[]{maiv}  {MAIV}   {Manufacturing, Assembly, Integration and Verification}
\newacronym[]{mal}{MAL} {\acrshort{cii} Middleware Abstraction Layer}
\newacronym[]{map}{MAP} {maximum a posteriori (reconstructor) }
\newacronym[]{mas} {mas}  {milli-arcsecond}
\newacronym[]{mcao}{MCAO} {Multi-Conjugate Adaptive Optics}
\newacronym[]{mcdram}{MCDRAM} {Multi-Channel DRAM}
\newacronym[]{metis}{METIS} {Mid-infrared ELT Imager and Spectrograph}
\newacronym[]{mf} {MF}  {Matched Filters}
\newacronym[]{micado}{MICADO} {Multi-Adaptive Optics Imaging Camera for Deep Observations}
\newacronym[]{mir}{MIR}{mid-infrared}
\newacronym[]{mmac}{MMAC} {Multiply-Accumulate Operation}
\newacronym[]{mmse} {MMSE}  {minimum mean square error}
\newacronym[]{mpia}{MPIA} {Max Planck Institute for Astronomy}
\newacronym[]{modpwfs}{M\textsubscript{PWFS}} {PWFS model}
\newacronym[]{mpwfs} {MPWFS}  {modulated Pyramid Wavefront Sensor}
\newacronym[]{mrmon} {MR Monitor}  {Mis-Registration Monitor}
\newacronym[]{ms}  {MS}   {main structure} 
\newacronym[]{mtf}{MTF} {Modulation Transfer Function}
\newacronym[]{mtu}{MTU} {Maximum Transmission Unit}
\newacronym[]{mudpi}{MUDPI} {Multicast UDP Interface}
\newacronym[]{mv} {MV}  {minimum variance reconstructor}
\newacronym[]{mvm} {MVM}  {Matrix-Vector Multiplication}
\newacronym[]{m1}  {M1}   {ELT primary mirror}
\newacronym[]{m2}  {M2}   {ELT secondary mirror}
\newacronym[]{m3}  {M3}   {ELT tertiary mirror}
\newacronym[]{m4}  {M4}   {ELT quaternary mirror}
\newacronym[]{m4lcs} {M4LCS}   {ELT quaternary mirror Local Control System}
\newacronym[]{m5}  {M5}   {ELT tip-tilt field stabilisation mirror}
\newacronym[]{m6}  {M6}   {ELT folding mirror in the pre-focal station}

\newacronym[]{na}  {N/A}  {not applicable} 
\newacronym[]{ncpa} {NCPA} {Non-Common Path Aberration}
\newacronym[]{ngc} {NGC}  {New General detector Controller}
\newacronym[]{ngc2} {NGCII}  {New General detector Controller II \glsadd{NGCII}}
\newacronym[]{ngs} {NGS}  {Natural Guide Star}
\newacronym[]{nir} {NIR}  {near-infrared}
\newacronym[]{nova} {NOVA}  {Nederlandse Onderzoekschool Voor Astronomie}
\newacronym[]{numa} {NUMA}  {Non-Uniform Memory Access}

\newacronym[]{ob}  {OB}   {\gls{observation block}}
\newacronym[]{ocs}  {OCS}   {\gls{Observation Coordination System}}
\newacronym[]{ocm}  {OCM}   {Observation Coordination Manager (ICS application)}
\newacronym[]{octopus} {OCTOPUS}  {end to end Adaptive Optics Simulation tool}
\newacronym[]{od}  {OD}   {optical density}
\newacronym[]{oomao} {OOMAO}  {Object-oriented Matlab Adaptive Optics}
\newacronym[]{opd} {OPD}  {optical pathlength difference}
\newacronym[]{otf}  {OTF}   {Optical Transfer Function}
\newacronym[]{opcua}  {OPC/UA}   {Open Platform Communications / Unified Architecture}

\newacronym[]{paola} {PAOLA}  {Performance of Adaptive Optics for
Large (or Little) Apertures}
\newacronym[]{pbs} {PBS}  {Product Breakdown Structure}
\newacronym[]{pcb} {PCB}  {printed circuid board}
\newacronym[]{pcie} {PCIe}  {Peripheral Component Interconnect Express}
\newacronym[]{pcured} {P-CuReD}  {Pyramid WFS version of CuReD}
\newacronym[]{pdr} {PDR}  {Preliminary Design Review}
\newacronym[]{plc} {PLC}  {Programmable Logic Controller}
\newacronym[]{pfs} {PFS}  {Prefocal Station}
\newacronym[]{pi} {PI}  {Physik Instrumente}
\newacronym[]{picontrol} {PI}  {Proportional-Integral}
\newacronym[]{polc} {POLC}  {Pseudo-Open Loop Control}
\newacronym[]{pp} {PP}  {pupil plane}
\newacronym[]{pp3} {PP3}  {Pupil Plane 3}
\newacronym[]{ppc} {PPC}  {Pupil Position Control}
\newacronym[]{ppmon} {PP Monitor}  {Pupil Position Monitor}
\newacronym[longplural={power spectral densities}]{psd} {PSD}  {power spectral density}
\newacronym[]{psf} {PSF}  {point spread function}
\newacronym[]{psi} {PSI}  {Phase Sorting Interferometry}
\newacronym[longplural={Pseudo Synthetic Interaction Matrices}]{psim} {PSIM}  {Pseudo Synthetic Interaction Matrix}
\newacronym[]{psm} {PSM}  {pupil stabilisation mirror}
\newacronym[]{pt} {PT}  {pulse tube}
\newacronym[]{ptp} {PTP}  {Precision Time Protocol (IEEE-1588)}
\newacronym[]{pv} {PV}  {Peak to Valley}
\newacronym[]{pwfs} {P-WFS}  {Pyramid Wavefront Sensor}
\newacronym[]{pwv} {PWV}  {Precipitable Water Vapor}
\newacronym[]{pyps} {PYPS}  {Pyramid Phasing Sensor}
\newacronym[]{pyr} {PYR}  {Pyramid}


\newacronym[]{qacits} {QACITS}  {Quadrant Analysis of Coronagraphic Images for Tip-tilt Sensing}
\newacronym[]{qe}  {QE}   {Quantum Efficiency}

\newacronym[]{rad} {RAD}  {Rapid Application Development Toolkit}
\newacronym[]{ram} {RAM}  {Random-Access Memory}
\newacronym[]{rams} {RAMS}  {Reliability, Availability, Maintainability, Safety}
\newacronym[]{ravc} {RAVC}  {ring-apodized vortex coronagraph}
\newacronym[]{rap} {RAP}  {ring apodizer}
\newacronym[]{rbm} {RBM}  {Rigid Body Motion}
\newacronym[]{rdma} {RDMA}  {remote direct memory access}
\newacronym[]{recmat} {RM}  {reconstruction matrix}
\newacronym[]{rpc} {RPC}  {remote procedure call}
\newacronym[]{rf}{RF} {Reference Frame}
\newacronym[]{rfw}{RFW} {request for waiver}
\newacronym[longplural={reconstruction matrices}]{rm} {RM}  {reconstruction matrix}
\newacronym[]{rmcomp} {RM Composer}  {Reconstruction Matrix Composer}
\newacronym[]{rms} {rms}  {root mean square}
\newacronym[]{roe} {ROE}  {readout electronics}
\newacronym[]{roi} {ROI}  {Region of Interest}
\newacronym[]{ron} {RON}  {Read-Out Noise}
\newacronym[]{rous} {ROUS}  {Recurrent Optimisation of (M4) Unit's Stroke}
\newacronym[]{rtc} {RTC}  {Real-Time Computer} 
\newacronym[]{rtcolap}  {OLAP}   {Optical Linear Algebra Processor}
\newacronym[]{rtctk} {RTC Tk}  {ELT Instrument Adaptive Optics Real-Time Toolkit}
\newacronym[]{rtd} {RTD}  {Real-Time Display} 
\newacronym[]{rtf} {RTF}  {Rejection Transfer Function}
\newacronym[]{rtms} {RTMS}  {Real-Time MUDPI Stream Protocol}

\newacronym[]{saphira} {SAPHIRA}  {Leonardo SAPHIRA  near infrared HgCdTe eAPD array}
\newacronym[]{scao}{SCAO} {Single Conjugate Adaptive Optics}
\newacronym[]{sca} {SCA}  {SCAO Subsystem}
\newacronym[]{scaocs} {SCAO CS}  {SCAO Control System}
\newacronym[]{scapp1} {SCA PP1}  {Pupil Plane 1 of the SCAO Wavefront Sensor}
\newacronym[]{scapp2} {SCA PP2}  {Pupil Plane 2 of the SCAO Wavefront Sensor}
\newacronym[]{scafp1} {SCA FP1}  {Focal Plane 1 of the SCAO Wavefront Sensor}
\newacronym[]{scafp2} {SCA FP2}  {Focal Plane 2 of the SCAO Wavefront Sensor}
\newacronym[]{scexao} {SCExAO}  {Subaru Coronagraphic Extreme Adaptive Optics}
\newacronym[]{seq}{SEQ} {support equipment}
\newacronym[]{sfpdp}{SFPDP} {Serial Front Panel Data Port}
\newacronym[]{sfmon}{SF Monitor} {Subaperture Flux Monitor}
\newacronym[]{sh} {SH}  {Shack-Hartmann}
\newacronym[]{shwfs} {SH WFS}  {Shack-Hartmann Wavefront Sensor}
\newacronym[]{slao}{SLAO} {Single Laser Adaptive Optics}
\newacronym[]{simd}{SIMD} {Single instruction,  multiple data}
\newacronym[]{sim}{SIM} {synthetic interaction matrix}
\newacronym[]{snr} {SNR}  {Signal to Noise Ratio}
\newacronym[]{soa} {SOA}  {Service-Oriented Architecture}
\newacronym[]{sphere} {SPHERE}  {Spectro-Polarimetric High-contrast Exoplanet REsearch: extreme adaptive optics system and coronagraphic facility at the VLT}
\newacronym[]{sprint} {SPRINT}  {System Parameter Recurrent INvasive Tracking}
\newacronym[]{srtc} {SRTC}  {Soft Real-time Cluster}
\newacronym[]{sr} {SR}  {Strehl ratio}
\newacronym[]{svn} {SVN}  {Apache Subversion}
\newacronym[]{syssup} {SysSup}  {System Supervisor}
\newacronym[]{sw}  {SW}   {Software} 

\newacronym[]{tbc} {TBC}  {to be confirmed}
\newacronym[]{tbd} {TBD}  {to be defined} 
\newacronym[]{tcp} {TCP}  {Transmission Control Protocol}
\newacronym[]{tcs} {TCS}  {Telescope Control System}
\newacronym[]{tio} {TIO}  {Telescope and Instrument Operator}
\newacronym[]{tmt} {TMT}  {Thirty Meter Telescope}
\newacronym[]{trl} {TRL}  {technical readiness level}
\newacronym[]{tt}  {TT}   {Tip-Tilt}
\newacronym[]{ttm} {TTM}  {Tip-Tilt Mirror}
\newacronym[]{trs} {TRS}  {Time Reference System}
\newacronym[]{tvc} {TVC}  {temporal variance contrast}

\newacronym[]{udp} {UDP}  {User Datagram Protocol}
\newacronym[]{urd} {URD}  {User Requirements Document}
\newacronym[]{ut} {UT}  {VLT 8.2m Unit Telescope}

\newacronym[]{vc} {VC}  {Vortex Coronagraph}
\newacronym[]{vdm} {VDM}  {virtual deformable mirror}
\newacronym[]{vlt} {VLT}  {Very Large Telescope}
\newacronym[]{vlti} {VLTI}  {Very Large Telescope Interferometer}
\newacronym[]{vpm} {VPM}  {Vortex Phase Mask}

\newacronym[]{w2m}{W2M} {wavefront-to-mirror-modes function}
\newacronym[]{wcog}{wCoG} {Weighted CoG}
\newacronym[]{wcu}{WCU} {Warm Calibration UnitS}
\newacronym[]{wf} {WF}  {wavefront}
\newacronym[]{wfc} {WFC}  {Wavefront Control}
\newacronym[]{wfe} {WFE}  {wavefront error}
\newacronym[]{wfs} {WFS}  {Wavefront Sensor}
\newacronym[]{ws} {WS}  {Workstation}
\newacronym[]{wv} {WV}  {water vapor}
\newacronym[]{yao} {YAO}  {Yorick Adaptive Optics}



\longnewglossaryentry{telescope preset}
{
  name={telescope preset},
}
{%
The process during which the main axes of the telescope slew to a new target position or non-sidereal trajectory on sky to be tracked next.
In the context of the \gls{elt} ``a [telescope] preset is defined as a change in the telescope pointing by an angle larger than 60 arcsec on sky, i.e., larger than 60 arcsec in altitude and 56.4 arcsec in azimuth.'' \cite[Sec. 1.3.3]{ESO-253082_4}
}

\longnewglossaryentry{telescope offset}
{
  name={telescope offset},
}
{%
A command that changes the pointing of the telescope relative to the position or non-sidereal trajectory on sky defined by the telescope preset. 
}

\longnewglossaryentry{Active Optics}
{
  name={Active Optics},
}
{%
Controls the position and shape of the telescope's bulk optics in order to establish and maintain collimation. 
The correction bandwidth of Active Optics is low -- it is designed to deal with effects that vary slowly, such as flexure, or thermal contraction. 
In the context of the \gls{elt}, Active Optics components are controlled by ``\acrfull{loo}''.  
}

\longnewglossaryentry{Control System}
{
   name={Control System}
}
{%
from \cite{ESO-283831}:
``The ELT Control System architecture enforces a distinction between a telescope device or plant (e.g. the M2 unit, or the dome observing doors) and the component controlling that
device.

The controlling component is termed the Control System, while the device or plant is termed the System under Control.

As a system of systems, the ELT Control System contains layers of controllers. A lower level component comprising a Control System and System under Control appears as a System under Control to a higher level Control System.'' 

This definition also applies to the \gls{scaocs}.
}

\longnewglossaryentry{Differential tip-tilt}
{
   name={Differential tip-tilt control loop}
}
{%
A secondary wavefront control loop used for \gls{vc} observing modes. The \gls{qacits} algorithm is applied on \gls{fps} data to ensure that the star is centered on the \gls{vpm}.
}

\longnewglossaryentry{Differential high order}
{
   name={Differential high order control loop}
}
{%
A secondary wavefront control loop used for \gls{hci} observing modes. The \gls{psi} algorithm is applied on \gls{fps} and \gls{wfs} data to correct for \gls{ncpa} and water vapor seeing.
}



\longnewglossaryentry{Low Order Optimisation}
{
  name={Low Order Optimisation},
}
{%
A mode of operation, traditionally called ``\gls{Active Optics}''. The quasi-static aberrations of the telescope are observed at the Nasmyth adapter by Natural Guide Star probes and corrected by quasi-static adjustment of the mirror units position and mirror shape (when relevant). \cite[Sec. 1.3.3]{ESO-253082_4}
}

\longnewglossaryentry{guiding}
{
  name={guiding},
}
{%
Tracking using an error signal provided by devices measuring optically the pointing error on a reference star. \cite[Sec. 1.3.3]{ESO-253082_4}
}

\longnewglossaryentry{nodding}
{
  name={nodding},
}
{%
A process by way of which the projection of the field in the science focal plane is changed after, compared to chopping, longer intervals (minute time scales) by applying small offsets to the telescope pointing and keeping the relative position of the mirrors (both telescope and instrument) constant.
\cite[Sec. 2.1]{E-SPE-NOVA-MET-1030}
}



\longnewglossaryentry{Observation Coordination System}
{
  name={Observation Coordination System},
}
{%
The system responsible for observation coordination. It consists of the Observation Coordination Manager, Data Product Manager, one or more Subsystem Managers, zero or more Guiding Managers and the scripts implementing the scientific observation sequences.
}



\longnewglossaryentry{offsetting}
{
  name={offsetting},
}
{%
In the context of telescope kinematics, the process by way of which the pointing of the telescope is incrementally changed from one sky position to a nearby one. 
The \gls{elt} will realise all offsets larger than a small fraction of an arc second by acting on the telescope kinematics.
\cite[Sec. 1.3.3]{ESO-253082_4}
}

\longnewglossaryentry{plate scale}
{
  name={plate scale},
}
{%
The conversion factor between on-sky angular distances and on-detector linear scales.
The concept assumes that the underlying relation is linear, and plate scale is usually given in arc seconds (on-sky) per mm (on-detector). 
In practice, optical distortion is rarely zero and, depending on the desired level of fidelity, the transformation of object into image coordinates may require a polynomial expansion (with odd exponents only). 
In anamorphic systems, distortion may also vary differently along different axes of the image surface. 
\cite[Sec. 1.3.3]{ESO-253082_4}
}

\longnewglossaryentry{pointing}
{
  name={pointing},
}
{%
The actual direction the telescope is pointing (on-axis direction, defined by sky coordinates of the projection of the origin of the as-built coordinates system at the focus of the telescope).
\cite[Sec. 1.3.3]{ESO-253082_4}
}


\longnewglossaryentry{pointing error}
{
  name={pointing error},
}
{%
The difference between actual and required pointing.
\cite[Sec. 1.3.3]{ESO-253082_4}
}


\longnewglossaryentry{seeing}
{
  name={seeing},
}
{%
  Atmospheric seeing is the integrated, long-exposure effect of the atmospheric optical turbulence across the line of sight. When using Fried's model of free atmospheric seeing it is defined as seeing $= 0.98 \times \frac{\lambda}{r_0}$ where $\lambda$ is the optical wavelength and $r_0$ is the atmospheric coherence length. 
  Unless otherwise stated, seeing values in this document refer to those measured by the observatory astronomical site monitor at zenith and referenced to a wavelength of 0.5~µm.
  \cite[Sec. 1.3.3]{ESO-253082_4}

}

\longnewglossaryentry{seeing limited}
{
  name={seeing limited},
}
{%
  A mode of telescope operation in which the blind and \gls{loo} control of the telescope is complemented by an additional field stabilisation correction using the wavefront error signal from the telescope Natural Guide Star probes and correcting with the M4  adaptive mirror and the M5 fast tip-tilt mirror.
  \cite[Sec. 1.3.3]{ESO-253082_4}
}


\longnewglossaryentry{acquisition}
{
  name={acquisition},
}
{%
  The execution of a coordinated sequence of functions that prepares the system for a science exposure. In contrast to \gls{preset}, the motions are not blind and the involved sub-systems typically require receiving star light.

  \cite[Sec. 1]{ESO-302836}
}

\longnewglossaryentry{preset}
{
  name={preset},
}
{%
A commanded ”blind” motion of an actuator, or assembly of actuators, to a given position based on a specific input (Look-Up-Tables, coordinates, encoder position etc.). If not explicitly denoted differently, preset motions involving different sub-systems are supposed to be triggered and be carried out in parallel.
  \cite[Sec. 1]{ESO-302836_V3}
}

\longnewglossaryentry{observation block}
{
  name={observation block},
}
{%
The Observation Block is a pre-defined sequence of operations involving any combination of Telescope, Instrument and detector or data acquisition actions. The astronomer defines the parameters of this sequence prior to the observation run.
 \cite{ESO-288424}
}

\longnewglossaryentry{state}
{
  name={state},
}
{%
A descrition of the condition a system is in. To manage complexity a system is represented by a state machine, which defines a finite number of states. In the case of the \gls{elt} \gls{ics}, the three main states are foreseen: Off, Standby, and Operational. These are divided in a number of substates, such as initializing, acquisition, idle, etc. \cite[cf.][6.2.2.4]{ESO-205917}
}

\longnewglossaryentry{operational}
{
  name={operational},
}
{%
  A \gls{state} of a system \cite[cf.][Sec. 6.2.2.4]{ESO-205917}.
}

\longnewglossaryentry{pointing origin}
{
  name={pointing origin},
}
{%
The point in the focal plane which is associated with the target position on sky. If not derotated, the field appears to be rotating around the pointing origin. The pointing origin is expected to coincide with the projected center of the instrument's derotator.

}

\longnewglossaryentry{pointing reference}
{
  name={pointing reference},
}
{%
The expected position of the SCAO guide star in the focal plane, to which the SCAO Wavefront Control loop controls the pointing. When the instrument is in charge of the AO control it is the only spatially invariant point in the focal plane unless the derotator is tracking the field rotation. The pointing reference will be different from the \gls{pointing origin} for off-axis guide stars. 
} 



\longnewglossaryentry{rtcComputationTime}
{
  name={RTC computation time},
}
{%
Time elapsed between the first WFS data received at the \acrshort{rtc} and 
the last command data transmitted by the RTC~\cite{ESO-287130}.
}

\longnewglossaryentry{rtcLatency}
{
  name={RTC latency},
}
{%
Time elapsed between the last WFS data received at the \acrshort{rtc}
and the last command data sent by the \acrshort{rtc}~\cite{ESO-287130}.
}

\longnewglossaryentry{3rdPartySoftware}
{
  name={3rd party software},
}
{%
Any software not provided or standardised by ESO that is delivered to
ESO with the instrument and has not been developed internally, from the ground up by the
Instrument Consortium members directly subject to the ESO Instrument Contract
Statement of Work and ESO Intellectual Property requirements~\cite{ESO-287079_V2}.

The 3rd party SW therefore includes any SW developed as part of Instrument Consortium
external contracts and/or collaborations with legal entities other than ESO, as well as any
commercial SW product in use by the instrument not delivered or standardised by ESO.

The 3rd party SW includes as well any proprietary SW development environments (e.g.
compiler toolchains) subject to licensing costs and/or imposing a specific licensing
scheme to the products of the build~\cite{ESO-287079_V2}.
}

\longnewglossaryentry{openSourceSoftware}
{
  name={open source software},
}
{%
A software product is considered to be open source when its
source code is made available under a license in which the copyright holder provides the
end user with the right to use, study, modify and distribute the software~\cite{ESO-287079_V2}.
}


\longnewglossaryentry{scaomod}
{
  name={SCAO Module},
}
{%
The SCAO Module is part of the SCAO subsystem and contains the physical component parts involved in the Instrument's SCAO Wavefront Correction function, namely:
\begin{itemize}
 \item  Instrument's SCAO Wavefront Sensor (WFS), which measures in real-time the aberrations in the incoming wavefront to the Instrument.
%  \item [] [ ]
 \item Instrument's SCAO Auxiliary Actuators, used to bootstrap, maintain and optimise the SCAO Module optical configuration, and to compensate for wavefront aberrations developing in non-real-time. \cite[][Par. 79]{ESO-287079_V2}
\end{itemize} 
}

\longnewglossaryentry{pupil stabilisation mirror}
{
  name={Pupil Stabilization Mirror},
}
{%
A controllable tip-tilt mirror within the \gls{cfo}, very close to the \gls{cfo}-\gls{fp}1, which allows to control the lateral position of the reimaged pupil downstream of this component.
}

\longnewglossaryentry{field selector}
{
  name={Field Selector},
}
{%
A controllable tip-tilt mirror in the first pupil plane of the \acrfull{scaomod}, which allows to select the point in the field, which is centered on the \acrfull{wfs}. The AO guide star will be controlled to this pointing reference position. It can be located anywhere in the Field of View realized at the \acrshort{cfo} focal plane 1.
}


\longnewglossaryentry{derotator}
{
  name={Derotator},
}
{%
A K-Mirror in the common path of the \gls{cfo}, used to track the field or the pupil rotation for stable conditions downstream of the derotator.
}


\longnewglossaryentry{modulator}
{
  name={Modulator},
}
{%
A controllable tip-tilt mirror in the \gls{scapp2} of the \gls{scaomod}. Its task is to modulate the light of the AO guide star over the four facets of the pyramid. A sinusoidal tip-tilt motion of the mirror will cause the image of the star to move along a circular path around the tip of the pyramid with a frequency that corresponds to the integration time of the wavefront sensor.
}

\longnewglossaryentry{NGCII}
{
  name={NGCII},
}
{%
ESO`s detector controller that is being used for the \gls{elt} instruments.
}

